Simple yet Effective Node Property Prediction on Edge Streams under Distribution Shifts

The problem of predicting node properties (e.g., node classes) in graphs has received significant attention due to its broad range of applications. Graphs from real-world datasets often evolve over time, with newly emerging edges and dynamically changing node properties, posing a significant challenge for this problem. In response, temporal graph neural networks (TGNNs) have been developed to predict dynamic node properties from a stream of emerging edges. However, our analysis reveals that most TGNN-based methods are (a) far less effective without proper node features and, due to their complex model architectures, (b) vulnerable to distribution shifts. In this paper, we propose SPLASH, a simple yet powerful method for predicting node properties on edge streams under distribution shifts. Our key contributions are as follows: (1) we propose feature augmentation methods and an automatic feature selection method for edge streams, which improve the effectiveness of TGNNs, (2) we propose a lightweight MLP-based TGNN architecture that is highly efficient and robust under distribution shifts, and (3) we conduct extensive experiments to evaluate the accuracy, efficiency, generalization, and qualitative performance of the proposed method and its competitors on dynamic node classification, dynamic anomaly detection, and node affinity prediction tasks across seven real-world datasets.

==> 05_analysis.tex <==
\section{Complexity Analysis}
\label{sec:analysis}

We analyze the time complexity of \method ``in action'' after being trained. Specifically, we examine the cost of (a) updating the memory in response to a newly arrived edge, and (b) calculating anomaly scores for a query node.

\smallsection{Memory Update}
Given a newly arriving edge, \method updates the memory vector of each endpoint using GRU. 
The total time complexity is dominated by that  of GRU, which is $\calO({d_{s}}^{2}+d_{s}d_{m})$~\citep{rotman2021shuffling}, where $d_{s}$ and $d_{m}$ indicate the dimensions of memory vectors and messages respectively.

\smallsection{Anomaly Scoring}
Give a query node, \method first aims to restore its memory vector using TGAT with input being a zero-masked memory of the query node and the memory vectors of its at most $k$ most recent neighbors.
Thus, the time complexity of obtaining reconstructed memory is $\calO(k{d_{s}}^{2})$~\citep{zheng2023temporal} if we assume, for simplicity, that the embedding dimension of the attention layers is the same as the dimension $d_{s}$ of the memory vectors.
Then, \method computes the similarities (a) between the updated memory and previous memory vectors and (b) between retained and restored memory vectors, taking $\mathcal{O}({d_{s}}^{2})$ time.
As a result, the overall time complexity of \method for anomaly scoring of a node is $\mathcal{O}(k{d_{s}}^{2})$.

\red{Here, \method has the $\mathcal{O}(k{d_{s}}^{2}+d_{s}d_{m})$ time complexity which is constant with respect to the graph's growth (number of nodes and edges) per memory update and anomaly scoring.}
%Here, since all hyperparameters ($k, d_{s}$, and $d_{m}$) are constant, \method has the constant (i.e., $\mathcal{O}(1)$) time complexity per memory update and anomaly scoring.
If we perform anomaly scoring (for each endpoint) only when each edge arrives,
the total complexity is linear in the number of edges in the input CTDG so far.

==> 05_discussion.tex <==
\section{Discussion and Analysis}
\label{sec:dis&anlaysis}
In this section, we discuss how \method deals with various types of anomalies.
Then, we analyze the time complexity of \method.

\subsection{Discussion on Anomaly Types}
\label{sec:discussion}
Below, we discuss how \method can detect anomalies of various types, without any prior information about the types.
In Section~\ref{sec:exp:classification} (RQ4), we empirically confirm its effectiveness for all these types.


\smallsection{{T1) Hijacked Anomalies}}
This type involves a previously normal user's account being compromised at some point, exhibiting malicious behaviors that deviate from the user's normal pattern.
\method, motivated by such anomalies, contrasts short-term and long-term interaction patterns to spot them, as discussed above.



\smallsection{T2) New or Rarely-interacting Anomalies}
Many deep learning-based detection models struggle with anomalies involving (1) newly introduced or (2) rarely interacting nodes due to limited data for learning their normal behaviors.
\method assigns a higher anomaly score (both contrast and generation scores) to such nodes because their memory vectors undergo substantial changes until their long-term patterns are established.
We find it advantageous to pay attention to such nodes because, in some of the real-world datasets we used, including Wikipedia, Bitcoin-alpha, and Bitcoin-OTC, new and rarely interacting nodes are more likely to engage in anomalous actions than those with consistent interactions.\footnote{
We suspect that new or inactive accounts are typically used to perform anomalous actions since the cost of being suspended is low for such accounts.}


\smallsection{T3) Consistent Anomalies}
\label{disc:S1}
\method can also effectively identify anomalies exhibiting interaction patterns
that are consistent over time but deviating from those of normal nodes.
Due to the limited capacity (i.e., expressiveness) of the neural networks used in it, \method prioritizes learning prevalent patterns (i.e., those of normal nodes) over less common abnormal ones.
As a result, this can lead to a violation of \textbf{A2}, causing \method to assign high anomaly scores, especially memory generation scores, to such nodes.



\subsection{Complexity Analysis}
\label{sec:analysis}
We analyze the time complexity of \method ``in action'' after being trained. Specifically, we examine the cost of (a) updating the memory in response to a newly arrived edge, and (b) calculating anomaly scores for a query node.

\smallsection{Memory Update}
Given a newly arriving edge, \method updates the memory vector of each endpoint using GRU. 
The total time complexity is dominated by that  of GRU, which is $\calO({d_{s}}^{2}+d_{s}d_{m})$~\citep{rotman2021shuffling}, where $d_{s}$ and $d_{m}$ indicate the dimensions of memory vectors and messages respectively.

\smallsection{Anomaly Scoring}
Given a query node, \method first aims to generate its memory vector using TGAT with input being a zero-masked memory of the query node and the memory vectors of its at most $k$ most recent neighbors.
Thus, the time complexity of obtaining generated memory is $\calO(k{d_{s}}^{2})$~\citep{zheng2023temporal} if we assume, for simplicity, that the embedding dimension of the attention layers is the same as the dimension $d_{s}$ of the memory vectors.
Then, \method computes the similarities (a) between the current memory and previous memory vectors and (b) between current and generated memory vectors, taking $\mathcal{O}({d_{s}}^{2})$ time.
As a result, the overall time complexity of \method for anomaly scoring of a node is $\mathcal{O}(k{d_{s}}^{2})$.

The time complexity for both tasks is $\mathcal{O}(k{d_{s}}^{2}+d_{s}d_{m})$, which is \textbf{constant with respect to the graph size} (i.e., the numbers of accumulated nodes and edges).
If we assume that anomaly scoring (for each endpoint) is performed whenever each edge arrives,
the total complexity becomes linear in the number of accumulated edges, as confirmed empirically in Section~\ref{sec:exp:classification} (RQ2).

==> comparison.tex <==



% \begin{table*}
%     \vspace{-1mm}
%     \setlength{\tabcolsep}{5pt}
%     \centering
%     \small
%     \scalebox{1}{
%         \begin{tabular}{cccccccccccccc}
%             \toprule
%             $\calL_{n}$ & $\calL_{g}$ & $\calL_{m}$ & Cora-C & Citeseer & Pubmed & Cora-A & DBLP & Zoo & 20News & Mushroom & NTU2012 & ModelNet40 & A.R.$\downarrow$ \\
%             \midrule
%             \midrule
%             \ding{51}   & -         & -         & 80.23 $\pm$ 1.2       & 70.28 $\pm$ 1.5*      & 83.44 $\pm$ 0.6       & 81.94 $\pm$ 1.1       & 90.88 $\pm$ 0.1       & 79.94 $\pm$ 11.1      & \tb{80.18 $\pm$ 0.2}  & 99.76 $\pm$ 0.2       & 75.20 $\pm$ 2.6       & 97.01 $\pm$ 0.2       & 3.8       \\
%             -           & \ding{51} & -         & 79.69 $\pm$ 1.6       & 71.02 $\pm$ 1.3*      & 80.20 $\pm$ 1.3       & 78.98 $\pm$ 1.4       & 88.60 $\pm$ 0.2       & 79.31 $\pm$ 10.7      & 79.35 $\pm$ 0.4       & 99.13 $\pm$ 0.3       & 74.41 $\pm$ 2.6       & 96.66 $\pm$ 0.2       & 5.7       \\
%             -           & -         & \ding{51} & 76.76 $\pm$ 1.8       & 63.98 $\pm$ 2.0       & 79.86 $\pm$ 0.9       & 76.77 $\pm$ 1.1       & 63.95 $\pm$ 7.2       & 79.80 $\pm$ 11.0      & 79.27 $\pm$ 0.3       & 94.87 $\pm$ 0.7       & 73.11 $\pm$ 2.8       & 96.57 $\pm$ 0.2       & 6.9       \\
%             \ding{51}   & \ding{51} & -         & \ul{81.45 $\pm$ 1.2}  & 71.38 $\pm$ 1.4       & 83.68 $\pm$ 0.7       & \ul{82.00 $\pm$ 1.0}  & \ul{90.94 $\pm$ 0.1}  & 80.19 $\pm$ 11.1      & \tb{80.18 $\pm$ 0.2}  & \ul{99.81 $\pm$ 0.1}  & \tb{75.25 $\pm$ 2.5}  & 97.02 $\pm$ 0.1       & \ul{2.3}  \\
%             \ding{51}   & -         & \ding{51} & 80.49 $\pm$ 1.3       & 70.46 $\pm$ 1.5       & \ul{83.98 $\pm$ 0.7}  & 81.62 $\pm$ 1.0       & 90.75 $\pm$ 0.1       & 80.19 $\pm$ 11.1      & 80.15 $\pm$ 0.2       & 99.74 $\pm$ 0.2       & 75.12 $\pm$ 2.5       & \ul{97.03 $\pm$ 0.1}  & 3.6       \\
%             -           & \ding{51} & \ding{51} & 80.80 $\pm$ 1.1       & \ul{71.73 $\pm$ 1.4}  & 82.81 $\pm$ 0.7       & 80.24 $\pm$ 1.0       & 90.17 $\pm$ 0.1       & \ul{80.20 $\pm$ 11.1} & 79.29 $\pm$ 0.2       & 99.82 $\pm$ 0.1       & 73.76 $\pm$ 2.5       & 96.74 $\pm$ 0.1       & 4.1       \\
%             \ding{51}   & \ding{51} & \ding{51} & \tb{81.57 $\pm$ 1.1}  & \tb{72.02 $\pm$ 1.4}  & \tb{84.26 $\pm$ 0.6}  & \tb{82.15 $\pm$ 0.9}  & \tb{91.12 $\pm$ 0.1}  & \tb{80.25 $\pm$ 11.2} & 80.14 $\pm$ 0.2       & \tb{99.83 $\pm$ 0.1}  & \ul{75.23 $\pm$ 2.4}  & \tb{97.08 $\pm$ 0.1}  & \tb{1.4}  \\
%             \bottomrule
%         \end{tabular}
%     }
%     \normalsize
%     \vspace{-2mm}
%     \caption{Comparison of node classification accuracy according to whether or not to use each type of contrast (i.e., $\calL_{n}$, $\calL_{g}$, and $\calL_{m}$). %(i.e., node, hyperedge, and membership-level contrast) 
%     Using all types of contrasts (i.e., node-, group-, and membership-level contrast) achieves the best performance in most cases as they are complementarily reinforcing each other.
%     }
%     \label{tab:comparison}
%     \vspace{-3mm}
% \end{table*}


\begin{table*}
    % \vspace{-1mm}
    \setlength{\tabcolsep}{5pt}
    \setlength\aboverulesep{0.5pt}
    \centering
    \small
    \scalebox{1}{
        \begin{tabular}{ccccccccccc}
            \toprule
            $\calL_{n}$ & $\calL_{g}$ & $\calL_{m}$ & Cora-C & Citeseer & Pubmed & Cora-A & DBLP & NTU2012 & ModelNet40 & A.R.$\downarrow$ \\
            \midrule
            \midrule
            \ding{51}   & -         & -         & 80.23 $\pm$ 1.2       & 70.28 $\pm$ 1.5*      & 83.44 $\pm$ 0.6       & 81.94 $\pm$ 1.1       & 90.88 $\pm$ 0.1       & 75.20 $\pm$ 2.6       & 97.01 $\pm$ 0.2       & 4      \\
            -           & \ding{51} & -         & 79.69 $\pm$ 1.6       & 71.02 $\pm$ 1.3*      & 80.20 $\pm$ 1.3       & 78.98 $\pm$ 1.4       & 88.60 $\pm$ 0.2       & 74.41 $\pm$ 2.6       & 96.66 $\pm$ 0.2       & 5.6       \\
            -           & -         & \ding{51} & 76.76 $\pm$ 1.8       & 63.98 $\pm$ 2.0       & 79.86 $\pm$ 0.9       & 76.77 $\pm$ 1.1       & 63.95 $\pm$ 7.2       & 73.11 $\pm$ 2.8       & 96.57 $\pm$ 0.2       & 7       \\
            \ding{51}   & \ding{51} & -         & \ul{81.45 $\pm$ 1.2}  & 71.38 $\pm$ 1.4       & 83.68 $\pm$ 0.7       & \ul{82.00 $\pm$ 1.0}  & \ul{90.94 $\pm$ 0.1}  & \tb{75.25 $\pm$ 2.5}  & 97.02 $\pm$ 0.1       & \ul{2.3}  \\
            \ding{51}   & -         & \ding{51} & 80.49 $\pm$ 1.3       & 70.46 $\pm$ 1.5       & \ul{83.98 $\pm$ 0.7}  & 81.62 $\pm$ 1.0       & 90.75 $\pm$ 0.1       & 75.12 $\pm$ 2.5       & \ul{97.03 $\pm$ 0.1}  & 3.6       \\
            -           & \ding{51} & \ding{51} & 80.80 $\pm$ 1.1       & \ul{71.73 $\pm$ 1.4}  & 82.81 $\pm$ 0.7       & 80.24 $\pm$ 1.0       & 90.17 $\pm$ 0.1       & 73.76 $\pm$ 2.5       & 96.74 $\pm$ 0.1       & 4.4       \\
            \ding{51}   & \ding{51} & \ding{51} & \tb{81.57 $\pm$ 1.1}  & \tb{72.02 $\pm$ 1.4}  & \tb{84.26 $\pm$ 0.6}  & \tb{82.15 $\pm$ 0.9}  & \tb{91.12 $\pm$ 0.1}  & \ul{75.23 $\pm$ 2.4}  & \tb{97.08 $\pm$ 0.1}  & \tb{1.1}  \\
            \bottomrule
        \end{tabular}
    }
    \normalsize
    % \vspace{-2mm}
    \caption{Comparison of node classification accuracy according to whether or not to use each type of contrast (i.e., $\calL_{n}$, $\calL_{g}$, and $\calL_{m}$). %(i.e., node, hyperedge, and membership-level contrast) 
    Using all types of contrasts (i.e., node-, group-, and membership-level contrast) achieves the best performance in most cases as they are complementarily reinforcing each other.
    }
    \label{tab:comparison}
    % \vspace{-3mm}
\end{table*}

==> dataset.tex <==
\begin{table}[!t]
    \centering
    \scalebox{0.75}{
        \begin{tabular}{lcccc}
            \toprule
             & Wikipedia & Reddit & Bitcoin-alpha & Bitcoin-OTC \\
            \midrule
                \# Nodes             & 9,227  & 10,984     & 3,783     & 5,881  \\
                \# Edges        & 157,474  & 672,447     & 24,186     & 35,592   \\
                \# Features       & 172  & 172     & 0    & 0 \\
                \# anomalies    & 217   & 366      & 1520      & 4344        \\
                anomalies ratio    & 0.14\%   & 0.05\%      & 6.28\%      & 12.20\%        \\   
                anomaly type    & post ban   & edit ban      & Unreliable user      & Unreliable user        \\
            \bottomrule
        \end{tabular}
    }
    \caption{Statistics of datasets used in our experiments. The count of anomalies refers to the number of edges where the dynamic state of the actor node is abnormal, and the ratio represents the proportion of these abnormal edges in relation to the total number of edges.}
    \label{tab:dataset}
\end{table}

==> main_alg.tex <==
% \begin{figure}[t]
% \vspace{-2mm}
\begin{algorithm}[t]
\small
\caption{\generator: Transitive hypergraph generator\label{algo:generator}}
\KwIn{(1) Number of nodes $n$, hyperedge size distribution $S$ \newline 
(2) Community size $C$, intra-community hyperedge ratio $p$ \newline
(3) Level-sampling coefficient $\alpha$, level-size coefficient $\beta$}
\KwOut{Generated hypergraph $G' = (V', E')$}

% \state Initialize node index $idx=1$, level index $T = 1$, hash table $\Psi_{L}$, hyperedge set $E' = \emptyset$, and number of hyperedges $m = S.$size() \\ 
$idx \leftarrow 1$; $T \leftarrow 0$; $\Psi_L(T') \leftarrow \emptyset, \forall T' \in \mathds{N}^+$; $E' \leftarrow \emptyset$; $m \leftarrow \sum_k S(k)$ \\
$AE(1) \leftarrow 0$; $AE(i) \leftarrow 1, \forall i = \{2, \cdots, n\}$; $\Psi_{L}(0) \leftarrow \{v_{1}\} $ \label{line:nedgestart}\\ 
\While {$\operatorname{sum}(AE) < m$}{
$a \sim \operatorname{discrete-uniform}(\{2 , \cdots n\})$; $AE(a) \leftarrow AE(a) + 1$\label{line:nedgeend}\\ 
% $AE(a) \leftarrow AE(a) + 1$ where $a$ is sampled from $\{2 , \cdots n\}$ uniformly at random.
}

\While{$idx < n$}{   
    % \state $K \leftarrow T^{\beta} \times C$ \Comment{Number of new nodes in the current level}\label{line:newnodes}\\ 
    $T \leftarrow T + 1 $\Comment{{level in the hierarchy}}  \\
    $\Psi_{L}(T) \leftarrow\{v_{(idx + i)}\}_{1 \leq i \leq \min(CT^{\beta}, n - idx)}$ \label{line:currentlevel}
    \Comment{{node set at level $T$}} 
    \\
    \For {$i = 1 \ \textbf{to} \  \min (CT^{\beta}, n - idx) $}{
        $idx \leftarrow idx + 1$ \\ 
        \For {$j = 1 \ \textbf{to} \ AE(idx)$ }{
            $e' \leftarrow \{v_{idx}\}$; $s \sim S$; $q \sim \operatorname{uniform}(0, 1)$ \label{line:sample_prep} \\
            \If {$q$ < $p$} {
                $e'{\leftarrow}$ \textbf{\texttt{IntraCommunityGenerate}}($e'{,}idx{,}C{,}T{,}s{,}\Psi_{L}$) \\
                }
            \If {$\lvert e'\vert$ < s} {
                $e' \leftarrow$ \textbf{\texttt{HierarchicalGenerate}}($e', T, s, \Psi_{L}$)
                }
            $E' \leftarrow E' \cup \{ e' \}$
            }
        }
    }
\textbf{return} $G' = (V' = \{v_{1} , \cdots , v_{n}\}, E')$  \\ 
 \nlnonumber
\nonumber \hrulefill \\
\setcounter{AlgoLine}{0}
\nlnonumber
\SetKwProg{myproc}{\texttt{IntraCommunityGenerate}}{($e', {idx}, C, T, s, \Psi_L$)}{}~\label{subalgo:intracom}
  \myproc{}{
  ${idx'} = C \times \ceil[\big]{({idx}-2)/C} + 1$ \Comment{beginning index of community} \label{line:intracombeg}\\ 
  $V_{C} \leftarrow \Psi_L(T) \cap \{v_{({idx'} + 1)}, \cdots ,v_{({idx'} + C)}\} \setminus e'$ \label{line:intracomend}\Comment{community}\\
  % \Comment{community nodes} \\
  $V' \leftarrow $ uniformly sample $\min(s - 1, |V_C|)$ nodes from $V_{C}$ \\ 
  % $\min(\lvert V_{C}\vert , s - \lvert e'\vert)$ nodes from $V_{C}$ \\ 
  \Return $e' \cup V'$ \\
  }  
\setcounter{AlgoLine}{0}
\nlnonumber
\SetKwProg{myproce}{\texttt{HierarchicalGenerate}}{($e', T, s, \Psi_{L})$}{}~\label{subalgo:hier}
  \myproce{}{ 
  \While{$\lvert e'\vert < s$}{
    $\ell \leftarrow $ sample a level from $[0, 1, \cdots , T] $ proportional to $[\lvert \Psi_{L}(0)\vert, \alpha^{-1}\lvert \Psi_{L}(1)\vert , \cdots , \alpha^{-T}\lvert \Psi_{L}(T)\vert]$ respectively \label{line:firstsample}\\
    $v' \leftarrow $ sample a node from $\Psi_{L}(\ell)$ uniformly at random \label{line:secondsample}\\ 
    $e' \leftarrow e' \cup \{v'\}$
    }
    % \state \textbf{return} $e'$ \\
    \Return $e'$ \\
  }  
\end{algorithm}
% \end{figure}

==> main_complex.tex <==
\begin{table*}[t!]
\caption{Runtime (sec.) and memory consumption (MB) of five generators {for approximating} 12 real-world hypergraphs. 
{Note that \generator achieves the fastest generation time for all six hypergraphs with $\vert V \vert \geq 10^4$ (\textit{coauthorship} and \textit{q\&a}), and it exhibits the lowest memory consumption in four out of the six hypergraphs.
For each hypergraph, the best results are colored. `-' indicates that the generation process either exceeds the time limit of 12 hours or encounters an out-of-memory issue.}} \label{tab:gentimeandmemory}
    \centering
    \scalebox{0.75}{
    \renewcommand{\arraystretch}{0.92}
        \centering
        \begin{tabular}{c | c| c c c |c c c| c c |c c |c c | c}
            \toprule
            \multirow{2}{*}{\textbf{Statistic}} & \multirow{2}{*}{\textbf{Generator}} & \multicolumn{3}{c|}{coauthorship} & \multicolumn{3}{c|}{q\&a} & 
            \multicolumn{2}{c|}{email} & \multicolumn{2}{c|}{ndc} &  \multicolumn{2}{c|}{contact} & Average \\
            & & dblp & geology & history & ubuntu & math & server & enron & eu & classes & substances & high & primary & ranking \\
            \midrule
            \midrule
            \multirow{6}{*}{\makecell{\textbf{Runtime} \\ 
            \textbf{(sec.)}}} &\textbf{\generator} & \goat 4.07 & \goat 2.39 & \goat 1.86 & \goat 0.39 & \goat 0.33 & \goat 0.63 & 0.04 & 0.18 & 0.04 & \goat 0.09 & 0.10 & 0.18  & 1.7 \goat\\
            %\midrule
            \cmidrule{2-15}
            
            &\textbf{HyperPA}~\cite{do2020structural} & - & - & - & 374.51 & - & - & 5.02 & 5011.84 & 1155.00 & - & 2.29 & 4.56 & 5.0\\
            
            &\textbf{HyperFF}~\cite{ko2022growth} & 226.79 & 114.24 & 53.48 & 12.78 & 17.23 & 3.15 & 0.05 & \goat 0.09 & 0.32 & 0.10 & \goat 0.02 & \goat 0.02 & 2.7\\
            
            &\textbf{HyperLap}~\cite{lee2021hyperedges} & 19.07 & 9.57 & 2.24 & 0.57 & 0.45 & 1.14 & \goat 0.01 & 0.14 & \goat 0.01 & 0.10 & 0.06 & 0.04 & 1.8\\

            &\textbf{HyperLap+}~\cite{lee2021hyperedges} & 1322.6 & 611.91 & 160.75 & 12.08 & 1.00 & 23.46 & 0.06 & 2.74 & 0.29 & 3.92 & 0.26 & 0.51 & 3.7\\
            \midrule 
            \midrule 
            
            \multirow{6}{*}{\makecell{\textbf{Memory} \\ \textbf{consumption} \\ 
            \textbf{(MB)}}} &\textbf{\generator} & \goattwo 1535 & \goattwo 761 & \goattwo 325 & 90 & \goattwo 36 & 129 & 2 & 3 & \goattwo 2 & 11 & 11 & 23 & 2.0 \goattwo\\
            \cmidrule{2-15}

            &\textbf{HyperPA}~\cite{do2020structural} & - & - & - & \goattwo 21 & - & - & 76 & 60169 & 21351 & - & 2 & 2 & 4.2\\
            
            &\textbf{HyperFF}~\cite{ko2022growth} & 3307 & 1655 & 739 & 107 & 147 & \goattwo 26 & \goattwo 1 & \goattwo 2 & 4 & \goattwo 1 & \goattwo 1 & \goattwo 1 & 2.0 \goattwo \\
            
            &\textbf{HyperLap}~\cite{lee2021hyperedges} & 3197 & 1498 & 529 & 134 & 86 & 204 & 11 & 32 & 15 & 41 & 12 & 11 & 3.1\\
            
            &\textbf{HyperLap+}~\cite{lee2021hyperedges} & 5042 & 3005 & 1901 & 591 & 110 & 321 & 9 & 39 & 14 & 412 & 10 & 18 & 3.8\\
            
            \bottomrule
        \end{tabular}
        }
\end{table*}

==> main_res.tex <==
\begin{table*}[t!]
\vspace{-2mm}
\caption{Hypergraph transitivity $T(G)$ and D-statistic {between} hyperwedge transitivity $\mathcal{T}(w)$ distributions {in} the real-world hypergraphs and the generated ones.
% : Real-world, \generator, HyperCL, HyperFF, HyperLAP, and HyperLAP+. 
Among six generators, \generator reproduces $T(G)$ and distribution of $\mathcal{T}(w)$ most accurately.
%\textcolor{limegreen} cell implies minimum gap from real-world $T(G)$, and \textcolor{dodgerblue} cell implies minimum D-stat
The best reproduction results on each dataset are colored, and `*' indicates that the value is less than $10^{-3}$.
{`-' indicates that the generation process either exceeds the time limit of 12 hours or encounters an out-of-memory issue.}
} \label{tab:genobservation1}
\vspace{-1mm}
    \centering
    \scalebox{0.8}{
    \renewcommand{\arraystretch}{0.9}
        \centering
        \begin{tabular}{c | c| c c |c c |c c| c c c| c c c | c}
            \toprule
            \multirow{2}{*}{\textbf{Statistic}} & \multirow{2}{*}{\textbf{Generator}} &  \multicolumn{2}{c|}{email} & \multicolumn{2}{c|}{NDC} & \multicolumn{2}{c|}{contact} & \multicolumn{3}{c|}{coauthorship} & \multicolumn{3}{c|}{q\&a} & Average \\
            & & enron & eu & classes & substances & high & primary & dblp & geology & history & ubuntu & server & math  & ranking \\
            \midrule
            \midrule
            \multirow{7}{*}{\makecell{ \textbf{Hypergraph} \\ \textbf{transitivity} \\ \textbf{$T(G)$}}}&\textbf{Real World} & 0.195 & 0.125 & 0.052 & 0.019 & 0.345 & 0.336 & 0.007 & 0.005 & 0.002 & 0.005 & 0.005 & 0.025 & Real\\
            %\midrule 
            \cmidrule{2-15}
            
            &\textbf{\generator} & \goat 0.192 &  0.124 & \goat 0.052 & \goat 0.019 & \goat 0.344 & \goat 0.334 & \goat 0.007 & \goat 0.005 & \goat 0.002 & \goat 0.004 & \goat 0.004 & \goat 0.025  & \goat 1.08\\
            %\midrule
            \cmidrule{2-15}
            
            &\textbf{HyperCL}~\cite{lee2021hyperedges} & 0.078 & 0.053 & 0.008 & 0.005 & 0.119 & 0.223 & 0.000* & 0.000* & 0.000* & 0.014 & 0.017 & 0.040  &  4.08\\
            
            &\textbf{HyperPA}~\cite{do2020structural} & 0.090 & 0.110 & 0.070 & - & 0.121 & 0.153 & - & - & - & 0.003 & - & - & 4.75\\
            
            &\textbf{HyperFF}~\cite{ko2022growth} & 0.176 & \goat 0.125 & 0.006 & 0.003 & 0.006 & 0.007 & 0.047 & 0.048 & 0.048 & 0.051 & 0.050 & 0.054 &  4.83\\
            
            &\textbf{HyperLap}~\cite{lee2021hyperedges} & 0.123 & 0.085 & 0.008 & 0.008 & 0.220 & 0.301 & 0.001 & 0.000* & 0.000* & 0.016 & 0.015 & 0.004 & 3.25\\

            &\textbf{HyperLap+}~\cite{lee2021hyperedges} & 0.231 & 0.144 & 0.026 & 0.016 & 0.322 & 0.338 & 0.042 & 0.019 & 0.005 & 0.029 & 0.023 & 0.007 & 3.54\\
            \midrule 
            \midrule 
            
            \multirow{6}{*}{\makecell{\textbf{D-Statistic from} \\ \textbf{real-world $\mathcal{T}(w)$} \\ 
            \textbf{distribution}}} &\textbf{\generator} & 0.137 & 0.186 & 0.208 & 0.187 & \goattwo 0.101 & \goattwo 0.099 & \goattwo 0.111 & 0.197 & \goattwo 0.066 & 0.035 & 0.170 & 0.101 & \goattwo 2.25\\
            \cmidrule{2-15}
            &\textbf{HyperCL} & 0.285 & 0.285 & 0.395 & 0.482 & 0.372 & 0.243 & 0.239 & 0.385 & 0.113 & \goattwo 0.020 & 0.054 & 0.084 & 3.75 \\
            &\textbf{HyperPA}~\cite{do2020structural} & 0.235 & 0.319 & 0.410 & - & 0.360 & 0.319 & - & - & - & 0.034 & - & - & 5.25\\
            
            &\textbf{HyperFF}~\cite{ko2022growth} & \goattwo 0.094 & \goattwo 0.158 & 0.638 & 0.831 & 0.631 & 0.699 & 0.126 & \goattwo 0.131 & 0.290 & 0.354 & 0.215 & 0.087 & 3.75\\
            
            &\textbf{HyperLap}~\cite{lee2021hyperedges} & 0.191 & 0.178 & 0.369 & 0.326 & 0.223 & 0.124 & 0.150 & 0.265 & 0.089 & 0.021 & \goattwo 0.051 & \goattwo 0.051 & 2.50\\
            
            &\textbf{HyperLap+}~\cite{lee2021hyperedges} & 0.262 & 0.244 & \goattwo 0.175 & \goattwo 0.185 & 0.166 & 0.180 & 0.509 & 0.405 & 0.119 & 0.061 & 0.104 & 0.184 & 3.23\\
            
            \bottomrule
        \end{tabular}
        }
\end{table*}

==> tables/feature_selection_speed.tex <==


% \begin{figure*}[!h]
%     \begin{subfigure}{0.5\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/Wikipedia_ratio_test.png}
%         \caption{Wikipedia}
%         \label{fig:subfig1}
%     \end{subfigure}
%     \begin{subfigure}{0.5\textwidth}
%         \includegraphics[width=\textwidth]{figs/Reddit_ratio_test.png}
%         \caption{Reddit}
%         \label{fig:subfig2}
%     \end{subfigure}
%     \caption{ \label{fig:diagram}
%         The start point of test results.
%     }
%     % \vspace{-2mm}
% \end{figure*}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.48\textwidth]
    {figs/selection_speed_v3.png}
    \caption{ \label{fig:feature_selection_speed}
        Run time (in seconds) of the node feature selection based on general validation tuning with \model and proposed node feature selection in \method using one split time.
        The node features selected by both methods are identical. 
        Still, the linear model-based feature selection approach proposed in SPLASH shows superior efficiency compared to a general validation-based approach.
    }
\end{figure}

==> tables/synthetic_accuracy_new.tex <==

\begin{table}[t]
    \centering
    \vspace{-1.5mm}\caption{\label{tab:synthetic_performance} Performance (in \%) in the prediction of node properties in the synthetic datasets. %The synthetic datasets are split into 10/10/80$\%$ for the training, validation, and test sets. 
    %The first six methods are TGNN-based models, the next five methods are TGNN-based models utilizing random features as node features, and the next two methods are DTDG-based models. 
    For each dataset, the best and the second-best performances are highlighted in \textbf{boldface} and \ul{underlined}, respectively.
    \method performs best compared to other baselines under the artificial distribution shifts.
    %For results in terms of Average Precision (AP), refer to Online Appendix D.1.
    }
    \setlength{\tabcolsep}{2.5pt}
    %\setlength\aboverulesep{0.6pt}
    \small
    \scalebox{0.98}{
        \def\arraystretch{1.0}
        \begin{tabular}{@{}l|ccc}
        \toprule
         & \multicolumn{3}{c}{\textbf{Dynamic Node Classification}} \\ 
        & \multicolumn{3}{c}{\textbf{(F1 Score)}}  \\
         \cmidrule(lr){2-4} 
         & \textbf{Synthetic-50} & \textbf{Synthetic-70} & \textbf{Synthetic-90}  \\ \midrule
        JODIE~\cite{kumar2019predicting} & $10.15 \pm 0.13$ & $8.40 \pm 0.54$ & $5.37 \pm 0.87$ \\
        DySAT~\cite{sankar2020dysat} & $10.05 \pm 0.15$ & $11.25 \pm 3.79$ & $8.29 \pm 7.23$  \\
        TGAT~\cite{xu2020inductive} & $9.95 \pm 0.06$ & $8.59 \pm 3.57$ & $4.43 \pm 3.33$    \\
        TGN~\cite{tgn_icml_grl2020} & $10.13 \pm 0.30$ & $8.39 \pm 1.39$ & $4.64 \pm 1.12$  \\
        GraphMixer~\cite{cong2022we} & $10.03 \pm 0.18$ & $11.46 \pm 4.53$ & $12.91 \pm 9.35$  \\
        DyGFormer~\cite{yu2023towards} & $9.71 \pm 0.32$ & $8.59 \pm 4.65$ & $7.42 \pm 9.59$  \\
        \midrule
        JODIE+$RF$ & $10.22 \pm 0.37$ & $8.47 \pm 0.81$ & $8.17 \pm 1.02$   \\
        DySAT+$RF$ & $15.28 \pm 0.76$ & $13.72 \pm 0.23$ & $8.39 \pm 4.64$ \\
        TGAT+$RF$ & $20.06 \pm 0.04$ & $11.85 \pm 3.85$ & $7.96 \pm 4.53$  \\
        TGN+$RF$ & $18.26 \pm 1.99$ & $9.28 \pm 0.71$ & $8.50 \pm 1.36$   \\
        GraphMixer+$RF$ & $10.03 \pm 0.65$ & $10.82 \pm 4.39$ & $13.05 \pm 9.63$  \\
        DyGFormer+$RF$ & \ul{86.75 $\pm$ 0.15} & \ul{71.07 $\pm$ 8.86} & $14.16 \pm 8.01$   \\
        \midrule
        DIDA~\cite{zhang2022dynamic} & $30.79 \pm 1.45$ & $28.08 \pm 1.26$ & \ul{17.44 $\pm$ 1.66}   \\
        SLID~\cite{zhang2024spectral} & $31.69 \pm 6.71$ & $27.96 \pm 3.66$ & $15.89 \pm 4.28$   \\
        \midrule
        \textbf{\method} & \textbf{99.91 $\pm$ 0.10} & \textbf{99.97 $\pm$ 0.01} & \textbf{98.78 $\pm$ 0.59}  \\
        \bottomrule
        \end{tabular}
    }
\end{table}



